Orbeez-SLAM: A Real-time Monocular Visual SLAM with ORB Features and NeRF-realized Mapping

A spatial AI that can perform complex tasks through visual signals and cooperate with humans is highly anticipated. To achieve this, we need a visual SLAM that easily adapts to new scenes without pre-training and generates dense maps for downstream tasks in real-time. None of the previous learning-based and non-learning-based visual SLAMs satisfy all needs due to the intrinsic limitations of their components. In this work, we develop a visual SLAM named Orbeez-SLAM, which successfully collaborates with implicit neural representation and visual odometry to achieve our goals. Moreover, Orbeez-SLAM can work with the monocular camera since it only needs RGB inputs, making it widely applicable to the real world. Results show that our SLAM is up to 800x faster than the strong baseline with superior rendering outcomes. Code link: https://github.com/MarvinChung/Orbeez-SLAM.

==> sections/Introduction.tex <==
% 講一下visual SLAM 仍然是挑戰的，而且對於未來的美好映景有個更困難的需求(dense map, w/o PT, real time)，但前面的works都沒法滿足。

Simultaneous localization and mapping (SLAM) has drawn researchers' attention for decades. The visual SLAM is more challenging since it needs to receive visual signals (e.g., RGB-D images) rather than LiDAR or radar signals. Existing works reveal great success and are already applied to real-world applications such as sweeping robots. Besides, with the development of technology, an intelligent spatial AI that can receive visual signals and cooperate with humans to solve complicated tasks is highly valued. To achieve this, we need a visual SLAM that easily adapts to new scenes without pre-training and generates real-time fine-grained maps for downstream tasks.
% J: 可以提一下 downstream tasks 有哪些
However, previous visual SLAMs mainly focus on localization accuracy and only provide crude maps, which cannot satisfy our needs. Thus, we aim to develop a visual SLAM with the above properties.

% 除了nerf 之外想嘗試dense map的work，Tandem。導入Nerf，說她為什麼可能可以來生dense map.

 Recently, a representative learning-based visual SLAM, Tandem \cite{koestler2021tandem}, leverages the truncated signed distance function (TSDF) fusion to provide a dense 3D map. As claimed in \cite{koestler2021tandem}, Tandem achieves real-time inference and can work with a monocular camera. But, depth estimation is involved in the TSDF fusion, and the depth estimation module in Tandem needs pre-training before inference, which limits its adaptability to a novel scene significantly different from pre-trained scenes. In addition, Neural Radiance Field (NeRF) \cite{mildenhall2020nerf}, another implicit neural representation, does not require depth supervision during training and can be trained from scratch at the target scene. According to this attribute, using NeRF as the map in visual SLAM is a potential direction.

% 介紹那兩篇 Nerf-based SLAM, iMAP與NICE-SLAM。
Two latest NeRF-SLAMs \cite{Sucar:etal:ICCV2021, Zhu2022CVPR} echo our motivations. Among them, iMAP \cite{Sucar:etal:ICCV2021} is the first work that lets NeRF serve as the map representation in SLAM. Meanwhile, it also optimizes the camera pose via back-propagation from NeRF loss. Then, NICE-SLAM \cite{Zhu2022CVPR} extends iMAP and develops a hierarchical feature grid module. The module allows NICE-SLAM to scale up for large scenes without catastrophic forgetting. Nevertheless, the above NeRF-SLAM needs RGB-D images as inputs since they optimize camera pose purely through NeRF loss. In other words, they still need depth information to guide the 3D geometry, violating the intuition that NeRF can learn the scenes without depth. 

Besides, a notable shortcoming of NeRF is its slow convergence speed. Specifically, there are lots of rendering during the progress, which makes real-time training NeRF floundering. By observing this, instant-ngp \cite{mueller2022instant} compensates for the training speed issue. With the help of the multi-resolution hash encoding and the CUDA framework \cite{tiny-cuda-nn}, instant-ngp can train NeRFs in a few seconds. 

% 我們的work，動機、模型、數值結果。 圖一要扮演什麼角色?

% 貢獻總結


%Simultaneous localization and mapping (SLAM) is a well-known problem in robotics and computer vision. With the rise of embodied artificial intelligence (AI), robots may need to understand human perception. To solve such a problem, we require a real-time dense SLAM system and may need color information. Many recent works then combine deep learning on SLAM systems. Among these SLAM systems, monocular SLAM systems draw people's interest since they only need a monocular camera. Monocular real-time SLAM works \cite{yang20d3vo, koestler2021tandem} with deep learning relying on depth estimation from the neural network. The work Tandem \cite{koestler2021tandem} even provides dense 3D reconstruction with truncated signed distance function (TSDF) fusion while its depth estimation network requires offline training. The requirement of pretraining limits these deep learning SLAM systems' capability of adapting to new scenes. In the embodied AI situation, we would like robots capable of adapting to a new environment and retaining their performance. Therefore, we aim to produce a deep-learning SLAM without pretraining and generate a dense map.

%Neural Radiance Field (NeRF) \cite{mildenhall2020nerf} springs up in the computer vision area and shows its powerful capability in novel view synthesis. Since NeRF is a continuous function, it can fill the unseen region of the scene. This property makes NeRF a good representation of the map. The work iMAP \cite{Sucar:etal:ICCV2021} introduces using NeRF on the dense SLAM with the tracking and mapping pipeline. Since NeRF relies on the volume rendering \cite{468400}. Another work NICE-SLAM \cite{Zhu2022CVPR} extends the iMAP to scale up for larger scenes.  However, both works rely on RGB-D data which violates the intuition that NeRF only requires RGB data to train. 

%NeRF is notable for its long training time. NICE-SLAM \cite{Zhu2022CVPR}, an open-source NeRF-based SLAM, requires hours of training on the TUM dataset \cite{sturm12iros} which is not capable of real-time applications yet. The work instant-ngp \cite{mueller2022instant} compensates for the speed problem, with the help of the multi-resolution hash encoding and the CUDA framework \cite{tiny-cuda-nn}, the NeRF model can be trained in a few seconds. 

As depicted in Fig. \ref{fig:overview}, we seek to develop a SLAM system that trains NeRF with a monocular camera and achieves real-time inference for real-world applications. To this end, we introduce Orbeez-SLAM, a tracking and mapping pipeline that combines feature-based SLAM (e.g., ORB-SLAM2 \cite{murORB2}) and a NeRF working on the instant-ngp framework \cite{mueller2022instant}. Different from \cite{Sucar:etal:ICCV2021, Zhu2022CVPR}, we emphasize that the visual odometry (VO) (in ORB-SLAM2) can provide a better camera pose estimation even at the early beginning of the training, which let Orbeez-SLAM can be trained without depth supervision. Moreover, we simultaneously estimate camera poses via VO and update the NeRF-realized map. Notably, the training process is online and in real-time without pre-training. As a result, Orbeez-SLAM can render dense information such as the depth and color of scenes. Besides, it is validated in various indoor scenes and outperforms NeRF-SLAM baselines on speed and trajectory estimation aspects. To summarize, our contributions are threefold:

\begin{itemize}
    \item We rethink the benefits of visual odometry (VO). By combining VO with fast NeRF, our SLAM system reaches real-time inference and suits spatial AI applications.
    \item  Unlike existing NeRF-SLAM methods, our model does not need depth supervision.
    \item We develop Orbeez-SLAM, a pre-training-free system that adapts to novel scenes without delay. %with Our pretrain-free system is capable of adapting to a new environment from scratch in a very short time.

\end{itemize}



